Capacity ATL

Model checking strategic abilities was successfully developed and applied since the early 2000s to ensure properties in Multi-Agent System. In this paper, we introduce the notion of capacities giving different abilities to an agent. This applies naturally to systems where multiple entities can play the same role in the game, such as different client versions in protocol analysis, different robots in heterogeneous fleets, different personality traits in social structure modeling, or different attacker profiles in a cybersecurity setting. With the capacity of other agents being unknown at the beginning of the game, the longstanding problems of imperfect information arise. Our contribution is the following: (i) we define a new class of concurrent game structures where the agents have different capacities that modify their action list and (ii) we introduce a logic extending Alternating-time Temporal Logic to reason about these games.

==> lib/define.tex <==
\makeatletter
\newcommand{\DeclareLatinAbbrev}[2]{%
  \DeclareRobustCommand{#1}{%
    \@ifnextchar{.}{\textit{#2}}{%
      \@ifnextchar{,}{\textit{#2.}}{%
        \@ifnextchar{!}{\textit{#2.}}{%
          \@ifnextchar{?}{\textit{#2.}}{%
            \@ifnextchar{)}{\textit{#2.}}{%
              {\textit{#2.,\ }}}}}}}}%
}
\makeatother
\makeatletter
\newcommand{\DeclareLatinAbbrevNoComma}[2]{%
  \DeclareRobustCommand{#1}{%
    \@ifnextchar{.}{\textit{#2}}{%
      \@ifnextchar{,}{\textit{#2.}}{%
        \@ifnextchar{!}{\textit{#2.}}{%
          \@ifnextchar{?}{\textit{#2.}}{%
            \@ifnextchar{)}{\textit{#2.}}{%
              {\textit{#2.\ }}}}}}}}%
}
\makeatother
\DeclareLatinAbbrev{\eg}{e.g}
\DeclareLatinAbbrev{\Eg}{E.g}
\DeclareLatinAbbrev{\ie}{i.e}
\DeclareLatinAbbrev{\Ie}{I.e}
\DeclareLatinAbbrev{\etc}{etc}
\DeclareLatinAbbrevNoComma{\etal}{et~al}
\DeclareLatinAbbrev{\cf}{cf}
\DeclareLatinAbbrev{\st}{s.t}

% Tables
\AtBeginEnvironment{tabular}{\scriptsize}
%\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}

% Theorems
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

% General commands
\newcommand{\ceil}[1]{{\left \lceil{#1}\right \rceil}}
\newcommand{\floor}[1]{{\left \lfloor{#1}\right \rfloor}}
\newcommand{\brac}[1]{{\left\langle{#1}\right\rangle}}
\newcommand{\probability}[1]{{\mathbb{P}\left[{#1}\right]}}
\newcommand{\characteristic}[2]{{\mathds{1}_{#2}(#1)}}

% Environements

\newcommand{\examplename}{Example}


\newcommand{\parts}[1]{\mathcal{P}({#1})}
\newcommand{\partsOredered}[1]{\mathcal{P}_o({#1})}
\newtheorem{remark}{Remark}

% UPGS
\newcommand{\Nn}{\mathbb{N}}
\newcommand{\NnZero}{\mathbb{N}_0}
\newcommand{\upgs}{\mathcal{S}}
\newcommand{\player}{a}
\newcommand{\state}{q}
\newcommand{\capacity}{c}
\newcommand{\action}{\alpha}
\newcommand{\degree}{\delta}

\newcommand{\nbPlayers}{k}
\newcommand{\Players}{\mathbb{A}\mathsf{gt}}
\newcommand{\Capacities}{\mathsf{Cap}}
\newcommand{\states}{\mathsf{St}}
\newcommand{\labels}{\Pi}
\newcommand{\labeling}{\pi}
\newcommand{\actionVector}{\vec{\action}}
\newcommand{\Actions}{\mathsf{Act}}
\newcommand{\transition}{o}
\newcommand{\nbTransitions}{m}
\newcommand{\PlayerCapacitiesMapDef}{\Gamma}
\newcommand{\PlayerCapacitiesMap}[1]{\PlayerCapacitiesMapDef(#1)}
\newcommand{\capacityActionMapDef}{\gamma}
\newcommand{\capacityActionMap}[1]{\capacityActionMapDef(#1)}
\newcommand{\protocolDef}{d}
\newcommand{\protocol}[2]{\protocolDef_{#1}({#2})}
\newcommand{\upgsDef}{\brac{\Players, \Capacities, \states, \labels,
\labeling, \Actions, \PlayerCapacitiesMapDef, \capacityActionMapDef, \protocolDef,
\transition}}

\newcommand{\computation}{\rho}
\newcommand{\StateTrace}[1]{{#1}_{2\Nn -1}}
\newcommand{\ActionTrace}[1]{{#1}_{2\Nn}}
\newcommand{\history}{h}
\newcommand{\Paths}{\mathsf{Paths}}
\newcommand{\Histories}{\mathsf{Histories}}
\newcommand{\Outcomes}{\mathsf{Out}}
\newcommand{\strategy}{s}

% UPATL
\newcommand{\strat}[1]{\langle{#1}\rangle}
\newcommand{\nostrat}[1]{[{#1}]}
\newcommand{\hasCapacityDef}{\mapsto}
\newcommand{\hasCapacity}[2]{{#1} \hasCapacityDef {#2}}
%\newcommand{\nnext}{\ocircle}
\newcommand{\nnext}{\mathop{\mathcal{N}}}
%\newcommand{\always}{\Box}
\newcommand{\always}{\mathop{\mathcal{G}}}
%\newcommand{\eventually}{\Diamond}
\newcommand{\eventually}{\mathcal{F}}
\newcommand{\until}{\mathbin{\mathcal{U}}}
\newcommand{\releases}{\mathbin{\mathcal{R}}}
\newcommand{\knowsDef}{\mathcal{K}_{\textsf{cap}}}
\newcommand{\knows}[2]{\knowsDef^{#1}({#2})}
\newcommand{\might}[2]{\mathcal{M}_{\textsf{cap}}^{#1}({#2})}
\newcommand{\playerCoalition}{Y}
\newcommand{\assign}{x}
\newcommand{\assignCapacity}{\lambda}
\newcommand{\assignCapacitySet}{\mathbf{X}_{\mathsf{cap}}}
\newcommand{\assignCapacitySetFor}[1]{\assignCapacitySet^{#1}}
\newcommand{\assignStrategy}{\sigma}
\newcommand{\assignStrategySet}{\mathbf{X}_{\mathsf{str}}}
\newcommand{\assignStrategySetFor}[1]{\assignStrategySet^{#1}}
\newcommand{\dom}{\mathsf{dom}}
\newcommand{\knowledge}{\Lambda}
\newcommand{\assignAction}{\beta}
\newcommand{\assignActionSet}{\mathbf{X}_{\mathsf{act}}}
\newcommand{\assignActionSetFor}[1]{\assignActionSet^{#1}}

% Model checking
\newcommand{\capacityTransitionFunction}{\digamma}
\newcommand{\memoryFromHistoryDef}{M}
\newcommand{\memoryFromHistory}[1]{\memoryFromHistoryDef({#1})}
\newcommand{\memoryFromHistoryCoalition}[2]{\memoryFromHistoryDef_{#1}({#2})}
\newcommand{\MemorySetCoalition}[1]{\mathbf{\memoryFromHistoryDef}_{#1}}
\newcommand{\MemorySet}{\mathbf{\memoryFromHistoryDef}}
\newcommand{\mapIndex}{\kappa}
\newcommand{\funcInduction}{f}
\newcommand{\statesWithLastMemoryDef}{Q}
\newcommand{\statesWithLastMemory}[1]{\statesWithLastMemoryDef({#1})}
\newcommand{\statesWithLastMemoryCoalition}[2]{\statesWithLastMemoryDef_{#1}({#2})}
\newcommand{\Pre}{Pre}
\newcommand{\Succ}{Succ}
\newcommand{\pointedKnowledge}{\theta}
\newcommand{\PointedKnowledges}{\Theta}
\newcommand{\PointedKnowledgeIterate}{W}
\newcommand{\pointedKnowledgeFromFormula}[1]{\left[#1\right]}
\newcommand{\cgsDef}{\mathcal{C}}
\newcommand{\tail}[1]{\mathsf{tail}({#1})}
\newcommand{\countOc}[2]{\mathsf{cnt}({#1}, {#2})}
\newcommand{\sub}[1]{\mathsf{sub}({#1})}

% Other
\newcommand{\gab}[1]{{\color{blue}#1}}
\newcommand{\last}[1]{{#1}_{\{-1\}}}
\newcommand{\access}[2]{{#1}_{\{#2\}}}
\newcommand{\integerSet}[1]{[#1]}
\newcommand{\prefix}[2]{#1_{\integerSet{#2}}}
\newcommand{\pmapsto}{\rightharpoonup}
\newcommand{\hypothesis}[1]{\mathcal{H}_{#1}}

